Hash-Based Ray Path Prediction: Skipping BVH Traversal Computation by Exploiting Ray Locality

State-of-the-art ray tracing techniques operate on hierarchical acceleration structures such as BVH trees which wrap objects in a scene into bounding volumes of decreasing sizes. Acceleration structures reduce the amount of ray-scene intersections that a ray has to perform to find the intersecting object. However, we observe a large amount of redundancy when rays are traversing these acceleration structures. While modern acceleration structures explore the spatial organization of the scene, they neglect similarities between rays that traverse the structures and thereby cause redundant traversals. This paper provides a limit study of a new promising technique, Hash-Based Ray Path Prediction (HRPP), which exploits the similarity between rays to predict leaf nodes to avoid redundant acceleration structure traversals. Our data shows that acceleration structure traversal consumes a significant proportion of the ray tracing rendering time regardless of the platform or the target image quality. Our study quantifies unused ray locality and evaluates the theoretical potential for improved ray traversal performance for both coherent and seemingly incoherent rays. We show that HRPP is able to skip, on average, 40% of all hit-all traversal computations.

==> sections/poster/main.tex <==

%
% topics
%
\ccsdesc[300]{Computing methodologies~Ray tracing}
\ccsdesc[100]{Computing methodologies~Acceleration Structure}
\ccsdesc[300]{Hardware~Graphics Processing Units}
\ccsdesc[100]{Hardware~Predictor Table}
\printccsdesc  



%%%
%%% Figure 1
%%%
\begin{figure}[htb]
  \centering
  \includegraphics[width=.9\linewidth]{idea_wide}
  
  \caption{\label{fig:idea_wide} 
           BVH traversal algorithm extended with our HRPP predictor}
\end{figure}



\section{Introduction}

Ray tracing techniques~\cite{Whitted:1980:IIM:358876.358882} employ hierarchical acceleration structures, such as Bounding Volume Hierarchies (BVH), which capture the scene spatial locality through subdividing it into a hierarchy of ever tighter bounding boxes. Such acceleration structures reduce the amount of geometry that a ray has to intersect with at the cost of additional ray-box intersections, which have to precede ray-scene intersection computations. 


This work proposes and evaluates Hash-based Ray Path Prediction (HRPP), which aims to reduce the cost of traversing the BVH by exploiting ray coherence~\cite{Pharr:1997:RCS:258734.258791}, whereby rays from close-by origins and similar directions follow a similar path through the tree. HRPP exploits ray coherence present throughout a scene's traversal to skip redundant ray-box intersections.

\section{Hash-based Ray Path Prediction}

HRPP uses hardware structures to predict which nodes a ray is likely to intersect based on information gathered from previous rays.
As shown in Figure~\ref{fig:idea_wide}, HRPP defines a direct flow for rays to reach the acceleration structure's leaf nodes bypassing all interior nodes.

Rather than letting rays enter the acceleration structure via the ray pool, a fixed function hardware block computes a ray's hash value. The hash value of a ray is based on the ray's physical properties of origin and direction. The hash function associates a unique number with each ray to serve as a lookup index into HRPP's predictor table. 
The predictor table provides a mapping from unique ray hash values to node indices, which are used as pointers into the tree. 

Before any ray enters the tree, the ray's hash value is computed followed by a lookup in the predictor table. If the hash is present in the table a prediction for the ray is made. The prediction is then evaluated and if the evaluation results in a valid scene intersection, the traversal of all interior nodes is skipped. 


\section{Limit study}

%
% RESULT TABLE
%


\begin{table}[t]
\centering
\begin{tabular}{ |c||c|c|c|c|  }
 \hline
 Scene & \pbox{20cm}{hit-any \\ savings(\%)} & size (MB) & \pbox{20cm}{closest-hit \\ savings(\%)} & size (MB) \\
 \hline
 Teapot       & 4 & 16 & 69 & 2 \\
 Killeroo     & 48 & 10.8 & 52 & 84 \\
 Buddha       & 23 & 18 &  41 & 18 \\
 Sportscar    & \textless1 & 21 & 32 & 18 \\
 \hline
\end{tabular}
\caption{Evaluation of test scenes - resolution 1024x1024 - 8 spp - go up level 0 - hash precision 6}
\label{tab:table_label}
\end{table}


We extended PBRT~\cite{Pharr:2010:PBR:1854996} to evaluate HRPP's potential using five scenes with unique BVH of different geometrical and illumination complexities. Our results are summarized in Table ~\ref{tab:table_label}.

Results show that for scenes with highly complex lighting models it is very hard to predict illumination rays. While HRPP saves some computations, it achieves a less than 1\% prediction ratio for complex scenes. On the other hand, with geometrically complex scenes with simple lighting, e.g., the Buddha scene, we skip 30\% of all hit-any rays. HRPP's performs well on closest-hit prediction, on average 30\% of all interior nodes are skipped.
